Reducing complexes in multidimensional persistent homology theory

The Discrete Morse Theory of Forman appeared to be useful for providing filtration-preserving reductions of complexes in the study of persistent homology. So far, the algorithms computing discrete Morse matchings have only been used for one-dimensional filtrations. This paper is perhaps the first attempt in the direction of extending such algorithms to multidimensional filtrations. Initial framework related to Morse matchings for the multidimensional setting is proposed, and a matching algorithm given by King, Knudson, and Mramor is extended in this direction. The correctness of the algorithm is proved, and its complexity analyzed. The algorithm is used for establishing a reduction of a simplicial complex to a smaller but not necessarily optimal cellular complex. First experiments with filtrations of triangular meshes are presented.

==> correctm.tex <==
% This file defines a few macros useful in team work on a paper or a book.
% The main purpose of the macros is to faciliate having simultanously two versions
% of selected fragments of text (old and new) with appropriate comments so that
% co-authors may think before deciding which version is better.
%
% To use these macros you must put this file in the directory where you keep
% the source files and add the following two lines
%
%\include{correctm}
%\showcomments
%
% at the beginnig of the main source file.
% If you want to compile the source file without any comments,
% just replace \showcomments by \hidecomments. In this case only the new versions
% will be used in the compiled text and all comments will be ommitted.
% This gives a possibility of looking at the clean text while still keeping
% the alternatives in the source file
%
% The \corrl macro
% ================
%
% The main macro is \corrl and it has the following syntax
%
% \corrl comment<<old_version||new_version>>
%
% Note that <<, || and >> are obligatory even if old_version or new_version are empty texts.
% The words 'comment', 'old_version', 'new_version',
% mark the places where you put your own text, i.e. these are parameters of the macro.
% The meaning of the parameters is
%
%     'comment'     - just a comment set in a non-standard font so that it clearly differs from
%                      the proper text
%     'old_version' - here you put the old text, which you want replaced with the new text
%     'new_version' - here you put the new text
%
% If comments are turned on by \showcomments, you will see the comment, then the old version
% clearly seperated form the new version and a margin mark. If comments are turned off, you
% will see only the new version with no comments or marks.
%
% If comment, old_version and/or new_version are longer than one line, a good idea is
% to write this macro (as well as the following macros) as
% \corrl
%   comment
% <<
%   old_version
% ||
%   new_version
% >>
%
%
% The \corrq macro
% ================
%
% Another possibility is that you feel some fragment should be changed but you do not know what
% should be the new version. Then use the macro
%
%  \corrq comment<<questioned_text>>
%
% With comments turned on you will see the comment followed by the clearly marked
% questioned text
%
% The \corre macro
% ================
%
% Sometimes the new version is an almost obvious change, so you
% want the old version only in the source
% file (just in case ...) but not in the compiled file.
% Then use the macro
%
% \corre comment<<old_version||new_version>>
%
% which in the compiled file shows only the new version and the margin mark to indicate that
% changes were made.
%
% The \corrs macro
% ================
%
% When the change is almost obvious and short, use the macro
%
% \corrs comment<<old_version||new_version>>
%
% which is similar to the previous but automaticallly adds a comment
% old_version->new_version on the margin
%
% The \corrn and \corro macros
% ============================
%
% To settle matters you can use two more macros with the same syntax as \corrl
%
%  \corro - to force the old version - the new version and all comments are disregarded
%                                      (but present in the source file)
%  \corrn - to force the new version - the old version and all comments are disregarded
%                                      (but present in the source file)
%
% This is simple in use (just replace l, q or s in the macro name by o or n) but leaves rubbish
% in the source file. If you find ourselve using plenty of this stuff one can easily write a simple PERL
% script which will automatically remove all this rubbish.
%
%
% The \corrc macro
% ================
%
% This is to place in the source file a comment only. The syntax is
%
% \corrs comment <<>>
%
% Parameters containing whole paragraphs
% ======================================
%
% Note: the standard TeX macros cannot be called with parameters which go across paragraphs
% (i.e. contain \par or an empty line). However, there is a special mechanism which allows for that.
% It is implemented here in the form of alternative macros \longcorrl, \longcorrq, \longcorrs and so on.
% Since TeX better recovers from errors if such macros are not present, use them only when necessary.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macro definitions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\def\corcommstyle{\bf\tiny}
\def\corcommstyle{\bf\small\tt}

%This macro is to be used when an alternative approach is to be displayed
%versus the old approach

\def\corrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$OLD$<<$} \end{quote}
  #2
  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
  #3
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #3
 \fi
}

\long\def\longcorrl #1<<#2||#3>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$OLD$<<$} \end{quote}
  #2
  \begin{quote} {\corcommstyle ==NEW== } \end{quote}
  #3
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #3
 \fi
}


%This macro is to be used when there is some confusion
%No new text is proposed

\def\corrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  #2
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

\long\def\longcorrq #1<<#2>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}\\$<<$BEG$<<$} \end{quote}
  #2
  \begin{quote} {\corcommstyle $>>$END$>>$ } \end{quote}
 \else
  #2
 \fi
}

%This is just to introduce a comment

\def\corrc #1<<>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$COMMENT$>>$ #1\marginpar{!!}} \end{quote}
\fi
}

%This macro is intended for some evident corrections.
%Only the new text is displayed.
%Comment is typed on the margin.

\def\corre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

\long\def\longcorre #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #1}
 \else
  #3
 \fi
}

%This macro is intended to mark corrections to short simple typos.
%Only the new text is displayed and an automatic typo change is
%marked on the margin.

\def\corrs #1<<#2||#3>>{
\if\visiblecomments y
  #3\marginpar{\corcommstyle #2 $\rightarrow$ #3\\ #1}
 \else
  #3
 \fi
}

%The next two macros are to help settle the matters.
%Changing \corrx where x is l,q or s to \corro (\corrn)
%will result in just choosing the old (new) text.
%This is intended to provide a simple way to get rid of
%any comments, i.e. to "clean" the paper.
%Unfortunately the no longer needed versions remain
%in the source file so in the future it would be
%useful to have some preprocessor to clean also
%the source file.
%Note that since \corrq does not provide any new stuff
%it makes sense only to change it to \corro unless some
%new text is added later on.

\def\corro #1<<#2||#3>>{
#2}

\def\corrn #1<<#2||#3>>{
#3}

\long\def\longcorro #1<<#2||#3>>{
#2}

\long\def\longcorrn #1<<#2||#3>>{
#3}

% This macro is to hide in official version pieces of text
% which is not available for presentation yet.

\long\def\underconstruction #1<<<#2>>>{
\if\visiblecomments y
  \begin{quote} {\corcommstyle $<<$UNDER CONSTRUCTION - BEGIN$>>$ #1\marginpar{!!}} \end{quote}
  #2
  \begin{quote} {\corcommstyle $>>$UNDER CONSTRUCTION - END$>>$ } \end{quote}
 \else
 \fi
}



% These two macros are to tourn on/off comments

\def\showcomments{
  \let\visiblecomments y
}

\def\hidecomments{
  \let\visiblecomments n
}


==> defs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{defn}[thm]{Definition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{ex}[thm]{Example}
\newtheorem{alg}[thm]{Algorithm}
\newtheorem{conj}[thm]{Conjecture}

\newenvironment{proof}{\noindent\textsc{Proof: }}{\hfill$\fbox{}$\par\medskip\par}

\newenvironment{aenum}{\begin{enumerate}
 \renewcommand{\theenumi}{\alph{enumi}}
 \renewcommand{\labelenumi}{(\theenumi)}}{\end{enumerate}}

%-------------------------------------------------------------------------------
% General Abbreviations (from SysEquDiff, ComHom and new)
%-------------------------------------------------------------------------------

\newcommand{\C}{{\mathbb C}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\N}{{\mathbb N}}

% use capital calligraphic letters for combinatorial sets and maps,
% classes of sets, etc,
% normal capital letters for real space subsets and for vector fields.

\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

\newcommand{\ba}{{\bf a}} % for vectors
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\be}{{\bf e}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
\newcommand{\br}{{\bf r}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}

\newcommand{\cl}{\mbox{\rm cl\,}}
\newcommand{\diam}{\mbox{\rm diam\,}}
\newcommand{\dist}{\mbox{\rm dist\,}}
\newcommand{\id}{\mbox{\rm id\,}}
\newcommand{\image}{\mbox{\rm im\,}} % image
\newcommand{\Inv}{\mbox{\rm Inv\,}}     % KM 17.4.02  for maximal invariant set
\newcommand{\oh}{\mbox{\rm oh\,}}
\newcommand{\rank}{\mbox{\rm rank\,}}
\newcommand{\sgn}{\mbox{\rm sgn\,}}
\newcommand{\emb}{\mbox{\rm emb\,}}
\newcommand{\floor}{\mbox{\rm floor\,}}
\newcommand{\ceiling}{\mbox{\rm ceil\,}}  % KM 16.3.02
\newcommand{\card}{\mbox{\rm card\,}}
\newcommand{\dom}{\rm dom}
\def\scal#1{\langle #1 \rangle}
\newcommand{\Int}{\mbox{\rm Int\,}} %for interior

\def\mapright#1{\stackrel{#1}{\longrightarrow}}
\def\mapleft#1{\stackrel{#1}{\longleftarrow}}
\def\mapdown#1{\Big\downarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapup#1{\Big\uparrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapne#1{\nearrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapse#1{\searrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapsw#1{\swarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}
\def\mapnw#1{\nwarrow\rlap{$\vcenter{\hbox{$\scriptstyle#1$}}$}}


%-------------------------------------------------------------------------------
% Specific abbreviations, from LatticeHight and ACDEK
%-------------------------------------------------------------------------------

\newcommand{\Ws}{W^{s}}
\newcommand{\Wu}{W^{u}}

\newcommand{\dis}{\displaystyle}
\newcommand{\rX}{\textcolor{red}{X}}
\newcommand{\dd}{ \partial _P f(Q)}
\newcommand{\f}{ $f : X \longrightarrow \R$ }
\newcommand{\mvmap}{\to \cP}   % new notation for mv map

\newcommand{\wup}{\overline{wrap}\,}         % for upper combinatorial wrap
\newcommand{\wlo}{\underline{wrap}\,}        % for lower combinatorial wrap
%\newcommand{\swrap}{\mbox{\texttt wrap}}         % for support of wraps
%\newcommand{\swup}{\overline{{\mbox{\texttt wrap}}}\;}
%\newcommand{\swlo}{\underline{{\mbox{\texttt wrap}}}\;}

\newcommand{\wrap}{wrap\,} % new command for wrap
\newcommand{\swrap}{\mbox{\rm wrap}\,}         % for support of wraps
\newcommand{\swup}{\overline{{\mbox{\rm wrap}}}\,}
\newcommand{\swlo}{\underline{{\mbox{\rm wrap}}}\,}

\newcommand{\bdy}{{\partial}} % topological boundary and boundary operator
\newcommand{\cbdy}{bd\,} % new command: combinatorial boundary, replaces wrap^*
\newcommand{\sbdy}{\mbox{\rm bd\,}} % new command: set boundary
\newcommand{\sd}{\mbox{\rm sd\,}} % new command: subdivision

\newcommand{\mcgs}{Morse connections graph }

\newcommand{\MCG}{Morse Connections Graph}
\newcommand{\MCGf}{MCG_{\fm}}
\newcommand{\fm}{f}
\newcommand{\Par}[1]{\left( #1 \right)}      % ( #1 )
\newcommand{\Brc}[1]{\left\{ #1 \right\}}    % { #1 }
\newcommand{\Brq}[1]{\left[ #1 \right]}      % [ #1 ]
\newcommand{\Abs}[1]{\left| #1 \right|}      % | #1 |
\newcommand{\st}{ \ \mid \ }
\newcommand{\conup}[2]{#1 \nearrow #2}
\newcommand{\condown}[2]{#1 \searrow #2}
\newcommand{\mcg}{Morse connections graph}

\newcommand{\St}{\mathrm{St}\,} % star
\newcommand{\cSt}{\mathrm{\overline{St}}\,} % closed star % I suggest no to use it, TK.
\newcommand{\uSt}{\mathrm{St^+}\,} % upper star
\newcommand{\lSt}{\mathrm{St^{-}}\,} % lower star
\newcommand{\Lk}{\mathrm{Lk}\,} % link
\newcommand{\uLk}{\mathrm{Lk^+}\,} % upper link
\newcommand{\lLk}{\mathrm{Lk^{-}}\,} % lower link

\def\op#1{\stackrel{\circ}{#1}}

%-------------------------------------------------------------------------------
% New for special interpolations and mesuring functions from CEFKL
%-------------------------------------------------------------------------------

%\newcommand{\aphi}{{\varphi^\rceil}}
\newcommand{\aphi}{{\varphi^\urcorner}} % axis-wise phi
\newcommand{\apsi}{{\psi^\urcorner}} % axis-wise psi

\newcommand{\lphi}{{\overline{\varphi}}} % linear phi
\newcommand{\lpsi}{{\overline{\psi}}} % linear psi

\newcommand{\mphi}{{\tilde{\varphi}}} % continuous measuring phi
\newcommand{\mpsi}{{\tilde{\psi}}} % continuous measuring psi

\newcommand{\dm}{\mathrm{D}\,} % generic distance
\newcommand{\dmm}{\mathrm{D_m}\,} % matching distance
%\newcommand{\dtmm}{\mathrm{\widetilde{D}_m} % approximate matching distance

%-------------------------------------------------------------------------------
% New for AKL
%-------------------------------------------------------------------------------

\newcommand{\ma}{\texttt{m}\,} % for a matching function from A to B.
\newcommand{\re}{\texttt{r}\,} % for the inverse matching from B to A. If you don't like this, an alternative is just m and r. TK


\newcommand{\sS}{\texttt{S}} % for sets of cells and canonical bases of chain complexes related to partition. 
\newcommand{\sA}{\texttt{A}} 
\newcommand{\sB}{\texttt{B}}
\newcommand{\sC}{\texttt{C}} % the set of critial cells
\newcommand{\sD}{\texttt{D}} % appears in the algorithm
\newcommand{\sM}{\texttt{M}} % future use: the set of basic cells of the Morse complex. A standard choice for bases is capital calligraphic letters, e.g. $\cS$, which is an alternative, but $\cS$ will suit the algorithm style. TK

\newcommand{\mI}{\texttt{$\max\!$I}\,}




